Structure and Behaviour of Virtual Organisation Breeding Environments

This paper provides an outline of a formal approach that we are developing for modelling Virtual Organisations (VOs) and their Breeding Environments (VBEs). We propose different levels of representation for the functional structures and processes that VBEs and VOs involve, which are independent of the specificities of the infrastructures (organisational and technical) that support the functioning of VBEs. This allows us to reason about properties of tasks performed within VBEs and services provided through VOs without committing to the way in which they are implemented.

==> eptcsdata.tex <==
\providecommand{\event}{Jeremy W. Bryans and John S. Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2009 (FAVO2009)}
\providecommand{\volume}{16}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{26}
\providecommand{\eid}{3}
\pdfoutput=1

